Few-shot Text Classification with Distributional Signatures

In this paper, we explore meta-learning for few-shot text classification. Meta-learning has shown strong performance in computer vision, where low-level patterns are transferable across learning tasks. However, directly applying this approach to text is challenging--lexical features highly informative for one task may be insignificant for another. Thus, rather than learning solely from words, our model also leverages their distributional signatures, which encode pertinent word occurrence patterns. Our model is trained within a meta-learning framework to map these signatures into attention scores, which are then used to weight the lexical representations of words. We demonstrate that our model consistently outperforms prototypical networks learned on lexical knowledge (Snell et al., 2017) in both few-shot text classification and relation classification by a significant margin across six benchmark datasets (20.0% on average in 1-shot classification).

==> examples/fig-grandma.tex <==
\begin{table}[t!]
    \small
	\renewcommand{\hlr}[2]{\setlength{\fboxsep}{.3pt}\colorbox{red!#2}{\rule[-1mm]{0pt}{3.5mm}{#1}}}
	\centering
	\begin{tabular}{p{0.87\linewidth}}
		%\toprule
		\emph{Prototypical network (seen class)}\\
		%\arrayrulecolor{grey}  % choose color
		\midrule
		\hlr{this}{3} \hlr{gorgeous}{10} \hlr{grandma}{100} \hlr{proves}{6} \hlr{beauty}{27} \hlr{has}{5} \hlr{no}{4} \hlr{expiration}{0} \hlr{date}{13}  \\
		\arrayrulecolor{black}
		\vspace{0.01cm}
		\emph{Prototypical network (unseen class)}\\
		\midrule
		\hlr{this}{4} \hlr{gorgeous}{7} \hlr{grandma}{12} \hlr{proves}{3} \hlr{beauty}{17} \hlr{has}{2} \hlr{no}{15} \hlr{expiration}{0} \hlr{date}{46}  \\
		\arrayrulecolor{black}
		\vspace{0.01cm}
		\emph{Our model (unseen class)}\\
		\midrule
		\hlr{this}{0} \hlr{gorgeous}{59} \hlr{grandma}{100} \hlr{proves}{3} \hlr{beauty}{32} \hlr{has}{0} \hlr{no}{1} \hlr{expiration}{0} \hlr{date}{10}  \\
	\end{tabular}
	\captionof{figure}{
      Visualization of word importance
      on an example from class \emph{fifty} in HuffPost headlines.
      %We compare the word importance predicted by
      %a prototypical network (\textsc{proto})~\citep{snell2017prototypical}
      %with our model.
      %We compare the magnitude of the CNN activations of
      %a prototypical network~\citep{snell2017prototypical}
      %and the attention generated by our model.
      %CNN activates on important features.
      Top: When \emph{fifty} is seen during meta-training,
      prototypical network~\citep{snell2017prototypical}
      recognizes important words.
      Middle: When \emph{fifty} is not available during meta-training,
      it fails to generalize.
      Bottom: Our model can identify salient words for unseen classes.
	}\label{fig:intro}
    \vspace{-4mm}
\end{table}


==> examples/fig-wpi.tex <==
{
\setlength{\tabcolsep}{10pt}
\begin{table*}[t!]
    \small
	\centering
	\begin{tabular}{p{0.45\linewidth} p{0.45\linewidth}}
		%\toprule
		\emph{\textsc{Ours}}\\
		%\arrayrulecolor{grey}  % choose color
		\midrule
		\hlr{s.}{0} \hlr{korean}{0} \hlr{wholesale}{100} \hlr{prices}{0} \hlr{up}{0} \hlr{0.4}{0} \hlr{pct}{0} \hlr{in}{0} \hlr{may}{0} \hlr{south}{0} \hlr{korea}{0} \hlr{'s}{0} \hlr{wholesale}{16} \hlr{price}{0} \hlr{index}{0} \hlr{,}{0} \hlr{base}{0} \hlr{1980}{0} \hlr{,}{0} \hlr{rose}{0} \hlr{0.4}{0} \hlr{pct}{0} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{0} \hlr{a}{0} \hlr{1.1}{0} \hlr{pct}{0} \hlr{rise}{0} \hlr{in}{0} \hlr{april}{0} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{0} \hlr{pct}{0} \hlr{higher}{0} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{0} \hlr{of}{0} \hlr{korea}{0} \hlr{said}{0} \hlr{.}{0} 
        &
		\hlr{s.}{0} \hlr{korean}{28} \hlr{wholesale}{43} \hlr{prices}{1} \hlr{up}{0} \hlr{0.4}{2} \hlr{pct}{6} \hlr{in}{0} \hlr{may}{0} \hlr{south}{3} \hlr{korea}{26} \hlr{'s}{0} \hlr{wholesale}{100} \hlr{price}{1} \hlr{index}{14} \hlr{,}{0} \hlr{base}{3} \hlr{1980}{0} \hlr{,}{0} \hlr{rose}{0} \hlr{0.4}{0} \hlr{pct}{0} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{0} \hlr{a}{0} \hlr{1.1}{0} \hlr{pct}{0} \hlr{rise}{0} \hlr{in}{0} \hlr{april}{0} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{0} \hlr{pct}{0} \hlr{higher}{0} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{0} \hlr{of}{0} \hlr{korea}{0} \hlr{said}{0} \hlr{.}{0} \\
		\arrayrulecolor{black}
		\vspace{0.01cm}
		\emph{$\mathrm{s}(x)$}\\
		\midrule
		\hlr{s.}{0} \hlr{korean}{22} \hlr{wholesale}{59} \hlr{prices}{1} \hlr{up}{0} \hlr{0.4}{100} \hlr{pct}{0} \hlr{in}{0} \hlr{may}{0} \hlr{south}{7} \hlr{korea}{19} \hlr{'s}{0} \hlr{wholesale}{59} \hlr{price}{0} \hlr{index}{100} \hlr{,}{0} \hlr{base}{22} \hlr{1980}{26} \hlr{,}{0} \hlr{rose}{1} \hlr{0.4}{100} \hlr{pct}{0} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{1} \hlr{a}{0} \hlr{1.1}{42} \hlr{pct}{0} \hlr{rise}{2} \hlr{in}{0} \hlr{april}{0} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{26} \hlr{pct}{0} \hlr{higher}{5} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{1} \hlr{of}{0} \hlr{korea}{19} \hlr{said}{0} \hlr{.}{0}
		&
		\hlr{s.}{0} \hlr{korean}{45} \hlr{wholesale}{100} \hlr{prices}{2} \hlr{up}{0} \hlr{0.4}{32} \hlr{pct}{0} \hlr{in}{0} \hlr{may}{0} \hlr{south}{12} \hlr{korea}{37} \hlr{'s}{0} \hlr{wholesale}{100} \hlr{price}{1} \hlr{index}{14} \hlr{,}{0} \hlr{base}{14} \hlr{1980}{32} \hlr{,}{0} \hlr{rose}{1} \hlr{0.4}{32} \hlr{pct}{0} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{1} \hlr{a}{0} \hlr{1.1}{37} \hlr{pct}{0} \hlr{rise}{1} \hlr{in}{0} \hlr{april}{1} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{21} \hlr{pct}{0} \hlr{higher}{5} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{5} \hlr{of}{0} \hlr{korea}{37} \hlr{said}{0} \hlr{.}{0} \\
		\arrayrulecolor{black}
		\vspace{0.01cm}
		\emph{$\mathrm{t}(x)$}\\
		\midrule
		\hlr{s.}{0} \hlr{korean}{0} \hlr{wholesale}{14} \hlr{prices}{100} \hlr{up}{0} \hlr{0.4}{0} \hlr{pct}{5} \hlr{in}{0} \hlr{may}{0} \hlr{south}{0} \hlr{korea}{0} \hlr{'s}{0} \hlr{wholesale}{14} \hlr{price}{65} \hlr{index}{7} \hlr{,}{0} \hlr{base}{0} \hlr{1980}{0} \hlr{,}{0} \hlr{rose}{0} \hlr{0.4}{0} \hlr{pct}{5} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{0} \hlr{a}{0} \hlr{1.1}{0} \hlr{pct}{5} \hlr{rise}{0} \hlr{in}{0} \hlr{april}{2} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{0} \hlr{pct}{5} \hlr{higher}{2} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{0} \hlr{of}{0} \hlr{korea}{0} \hlr{said}{0} \hlr{.}{0}
		&
		\hlr{s.}{0} \hlr{korean}{0} \hlr{wholesale}{0} \hlr{prices}{0} \hlr{up}{0} \hlr{0.4}{0} \hlr{pct}{100} \hlr{in}{0} \hlr{may}{0} \hlr{south}{0} \hlr{korea}{0} \hlr{'s}{0} \hlr{wholesale}{0} \hlr{price}{0} \hlr{index}{0} \hlr{,}{0} \hlr{base}{0} \hlr{1980}{0} \hlr{,}{0} \hlr{rose}{0} \hlr{0.4}{0} \hlr{pct}{100} \hlr{to}{0} \hlr{127.0}{0} \hlr{in}{0} \hlr{may}{0} \hlr{after}{0} \hlr{a}{0} \hlr{1.1}{0} \hlr{pct}{100} \hlr{rise}{0} \hlr{in}{0} \hlr{april}{1} \hlr{and}{0} \hlr{was}{0} \hlr{1.5}{0} \hlr{pct}{100} \hlr{higher}{0} \hlr{than}{0} \hlr{in}{0} \hlr{may}{0} \hlr{1986}{0} \hlr{,}{0} \hlr{the}{0} \hlr{bank}{2} \hlr{of}{0} \hlr{korea}{0} \hlr{said}{0} \hlr{.}{0} \\
	\end{tabular}
	\captionof{figure}{
	  Task-agnostic attention weights,
      visualized for class ``wpi'' (wholesale price index).
      Left: fine-grained classification (wpi vs. other commerce-related classes).
      Right: coarse-grained classification (wpi vs. non-commerce classes).
      Top to bottom: our model's predictions, $\mathrm{s}(x)$, $\mathrm{t}(x)$ .
	}
	\label{fig:wpi}
    \vspace{-5mm}
\end{table*}
}


==> section/archive/tables.tex <==
\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{857} & \multicolumn{2}{c}{956}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $33.9512 \pm 0.3342$ & $45.8717 \pm 0.3926$ & $30.0954 \pm 0.1595$ & $39.7002 \pm 0.1384$ \\
IDF & NN &  $38.8810 \pm 0.3312$ & $51.9491 \pm 0.2057$ & $36.1192 \pm 0.3013$ & $47.1677 \pm 0.2225$ \\
\midrule
AVG & Proto &  $36.2525 \pm 0.3345$ & $45.4267 \pm 1.3674$ & $28.0397 \pm 0.6617$ & $36.6424 \pm 1.7547$ \\
IDF & Proto &  $37.8616 \pm 1.1332$ & $46.5373 \pm 1.4468$ & $29.3400 \pm 0.9352$ & $38.4091 \pm 0.6212$ \\
CNN & Proto &  $29.6754 \pm 1.0284$ & $35.0906 \pm 0.7165$ & $23.8141 \pm 0.8539$ & $27.6075 \pm 1.4730$ \\
\midrule
AVG & MAML &  $23.6877 \pm 1.8117$ & $23.6094 \pm 2.9175$ & $23.9490 \pm 1.0051$ & $23.3930 \pm 0.9831$ \\
IDF & MAML &  $27.5040 \pm 0.5852$ & $29.1077 \pm 1.3020$ & $26.4902 \pm 0.5256$ & $27.5118 \pm 1.0394$ \\
CNN & MAML &  $22.4792 \pm 0.7267$ & $23.0138 \pm 1.1195$ & $23.0104 \pm 0.4760$ & $23.6859 \pm 0.6949$ \\
\midrule
AVG & R2D2 &  $37.6056 \pm 0.1069$ & $57.2400 \pm 0.1998$ & $32.3757 \pm 0.2737$ & $50.4090 \pm 0.2492$ \\
IDF & R2D2 &  $44.8302 \pm 1.0704$ & $64.3515 \pm 0.5418$ & $40.7322 \pm 0.9323$ & $56.8224 \pm 1.2069$ \\
CNN & R2D2 &  $32.2502 \pm 1.6296$ & $44.3235 \pm 0.4445$ & $26.3776 \pm 0.8505$ & $35.1243 \pm 0.8393$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $50.0027 \pm 1.6315$ & $67.6720 \pm 0.2803$ & $45.1304 \pm 0.7436$ & $60.3709 \pm 0.4342$ \\
\multicolumn{2}{l}{Ours} &  $\bm{52.1776} \pm 0.6549$ & $\bm{68.3304} \pm 0.1792$ & $\bm{46.0827} \pm 1.3835$ & $\bm{61.7466} \pm 0.4997$ \\
\multicolumn{2}{l}{Ours+fuse} &  $50.9642 \pm 2.0569$ & $67.2942 \pm 1.0387$ & $46.2678 \pm 0.1292$ & $60.7634 \pm 1.2230$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $52.3435 \pm 1.1464$ & $67.9040 \pm 0.6025$ & $47.1458 \pm 0.3364$ & $60.7885 \pm 1.2830$ \\
\bottomrule
\end{tabular}
\centering
\caption{20newsgroup}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{easy} & \multicolumn{2}{c}{hard2}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $44.4994 \pm 0.2607$ & $58.7798 \pm 0.1552$ & $46.7678 \pm 0.1488$ & $60.3659 \pm 0.2029$ \\
IDF & NN &  $47.1914 \pm 0.1502$ & $64.0498 \pm 0.1469$ & $51.4322 \pm 0.1584$ & $67.1550 \pm 0.2141$ \\
\midrule
AVG & Proto &  $49.2014 \pm 0.9056$ & $60.1998 \pm 0.4867$ & $37.2680 \pm 1.8556$ & $51.9909 \pm 2.7298$ \\
IDF & Proto &  $51.5814 \pm 0.3760$ & $65.5976 \pm 0.9434$ & $41.9142 \pm 1.1749$ & $59.2411 \pm 1.1098$ \\
CNN & Proto &  $49.8488 \pm 0.7724$ & $56.4888 \pm 1.6452$ & $34.0203 \pm 1.4843$ & $44.4906 \pm 1.5391$ \\
\midrule
AVG & MAML &  $28.0355 \pm 0.4466$ & $32.0830 \pm 2.1638$ & $21.7499 \pm 0.7338$ & $24.2707 \pm 4.9296$ \\
IDF & MAML &  $29.2827 \pm 0.6503$ & $32.1005 \pm 0.6488$ & $30.4646 \pm 0.3215$ & $32.5842 \pm 1.8217$ \\
CNN & MAML &  $30.7616 \pm 1.6284$ & $35.2102 \pm 1.8281$ & $25.9861 \pm 0.2261$ & $27.6466 \pm 0.6006$ \\
\midrule
AVG & R2D2 &  $49.2429 \pm 0.4270$ & $71.1754 \pm 0.1618$ & $50.2539 \pm 0.2372$ & $72.7886 \pm 0.2371$ \\
IDF & R2D2 &  $57.3002 \pm 1.6229$ & $77.6378 \pm 0.0723$ & $60.2755 \pm 1.3370$ & $79.7896 \pm 0.2826$ \\
CNN & R2D2 &  $50.8867 \pm 0.2812$ & $62.5434 \pm 1.1333$ & $37.3090 \pm 0.8041$ & $53.8923 \pm 1.5403$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $58.7640 \pm 0.7626$ & $77.8981 \pm 0.1616$ & $61.7653 \pm 0.7250$ & $80.4461 \pm 0.1487$ \\
\multicolumn{2}{l}{Ours} &  $\bm{60.0445} \pm 0.5119$ & $\bm{78.9349} \pm 0.1637$ & $\bm{62.6611} \pm 0.6729$ & $\bm{81.1654} \pm 0.3171$ \\
\multicolumn{2}{l}{Ours+fuse} &  $60.5781 \pm 0.5452$ & $78.8715 \pm 0.2672$ & $62.2754 \pm 0.4413$ & $80.9219 \pm 0.2453$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $61.3445 \pm 0.2897$ & $79.5531 \pm 0.0643$ & $63.0862 \pm 0.6041$ & $81.2035 \pm 0.3069$ \\
\bottomrule
\end{tabular}
\centering
\caption{Amazon FastText}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{easy} & \multicolumn{2}{c}{hard}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $57.1011 \pm 0.2910$ & $71.0778 \pm 0.3211$ & $47.5842 \pm 0.3875$ & $60.6773 \pm 0.3005$ \\
IDF & NN &  $52.6685 \pm 0.2882$ & $68.7854 \pm 0.3234$ & $46.8498 \pm 0.3117$ & $60.6272 \pm 0.4112$ \\
\midrule
AVG & Proto &  $64.9035 \pm 1.0281$ & $65.5678 \pm 5.5935$ & $44.0461 \pm 0.8090$ & $46.5566 \pm 1.5877$ \\
IDF & Proto &  $63.7368 \pm 0.9935$ & $76.1394 \pm 0.9801$ & $43.0906 \pm 1.1544$ & $61.9952 \pm 1.8281$ \\
CNN & Proto &  $71.7331 \pm 0.7090$ & $80.1574 \pm 0.4183$ & $49.7899 \pm 0.2246$ & $65.1614 \pm 0.9934$ \\
\midrule
AVG & MAML &  $50.7210 \pm 6.0595$ & $66.1214 \pm 4.7212$ & $27.4134 \pm 1.2225$ & $32.3747 \pm 5.1963$ \\
IDF & MAML &  $62.8226 \pm 1.2447$ & $71.1309 \pm 0.6343$ & $34.2282 \pm 0.7491$ & $45.0496 \pm 1.2272$ \\
CNN & MAML &  $64.6930 \pm 0.2594$ & $72.2496 \pm 1.6190$ & $46.7979 \pm 2.0437$ & $58.9723 \pm 1.9261$ \\
\midrule
AVG & R2D2 &  $63.5598 \pm 0.8242$ & $77.3909 \pm 0.1293$ & $53.2512 \pm 1.0102$ & $72.2262 \pm 0.1613$ \\
IDF & R2D2 &  $62.3694 \pm 1.0157$ & $77.2909 \pm 0.7748$ & $55.6550 \pm 1.0888$ & $75.3026 \pm 0.3480$ \\
CNN & R2D2 &  $\bm{73.3861} \pm 0.2910$ & $82.4304 \pm 0.5038$ & $56.8373 \pm 2.3098$ & $71.8112 \pm 1.2586$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $71.0344 \pm 0.7823$ & $\bm{83.0254} \pm 0.1898$ & $66.8536 \pm 0.4648$ & $83.4230 \pm 0.1449$ \\
\multicolumn{2}{l}{Ours} &  $70.5715 \pm 0.9591$ & $81.5066 \pm 0.3090$ & $\bm{66.8955} \pm 0.6489$ & $\bm{83.5386} \pm 0.2712$ \\
\multicolumn{2}{l}{Ours+fuse} &  $71.5243 \pm 0.8695$ & $81.4102 \pm 0.9728$ & $67.5741 \pm 0.6149$ & $83.3462 \pm 0.5120$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $71.2899 \pm 0.9200$ & $81.5291 \pm 0.9277$ & $67.6077 \pm 0.5882$ & $83.4357 \pm 0.3219$ \\
\bottomrule
\end{tabular}
\centering
\caption{Fewrel FastText}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Hard}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $31.4517 \pm 0.1861$ & $41.5550 \pm 0.2348$ & $30.5922 \pm 0.1192$ & $39.2163 \pm 0.2518$ \\
IDF & NN &  $31.5398 \pm 0.1874$ & $42.3587 \pm 0.1581$ & $30.4874 \pm 0.1678$ & $40.1875 \pm 0.2141$ \\
\midrule
AVG & Proto &  $35.6832 \pm 1.2517$ & $41.6739 \pm 1.1323$ & $28.1856 \pm 0.5150$ & $36.7907 \pm 1.9820$ \\
IDF & Proto &  $34.8861 \pm 0.7357$ & $50.2451 \pm 0.9452$ & $28.2594 \pm 0.3426$ & $38.2621 \pm 0.5564$ \\
CNN & Proto &  $33.4981 \pm 0.7991$ & $44.2194 \pm 0.5873$ & $25.9400 \pm 0.6225$ & $31.9858 \pm 1.1052$ \\
\midrule
AVG & MAML &  $29.2773 \pm 1.2160$ & $37.2093 \pm 2.3099$ & $23.6829 \pm 0.2958$ & $27.0941 \pm 0.2866$ \\
IDF & MAML &  $34.3304 \pm 0.5381$ & $43.5768 \pm 0.4524$ & $25.4413 \pm 0.2995$ & $29.5680 \pm 0.3830$ \\
CNN & MAML &  $27.1133 \pm 0.9647$ & $33.5174 \pm 2.0138$ & $21.9950 \pm 0.1683$ & $24.4107 \pm 0.4018$ \\
\midrule
AVG & R2D2 &  $36.3381 \pm 0.3603$ & $54.8605 \pm 0.2148$ & $34.7734 \pm 0.2322$ & $50.7544 \pm 0.2543$ \\
IDF & R2D2 &  $37.6811 \pm 0.9615$ & $59.5626 \pm 1.7803$ & $36.3898 \pm 0.8689$ & $56.7907 \pm 0.2814$ \\
CNN & R2D2 &  $37.3229 \pm 1.1592$ & $49.9686 \pm 0.2025$ & $27.8752 \pm 0.1827$ & $36.6678 \pm 0.4769$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$}  &  $41.5586 \pm 0.5027$ & $61.2448 \pm 0.2060$ & $39.5416 \pm 0.2458$ & $57.0267 \pm 0.3392$ \\
\multicolumn{2}{l}{Ours}  &  $\bm{42.8278} \pm 0.5046$ & $\bm{63.5101} \pm 0.1098$ & $\bm{40.3845} \pm 0.1562$ & $\bm{58.8942} \pm 0.3378$ \\
\multicolumn{2}{l}{Ours+fuse} &  $43.6712 \pm 0.3073$ & $63.6666 \pm 0.1636$ & $40.1917 \pm 0.4247$ & $58.8038 \pm 0.3972$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $43.6587 \pm 0.2632$ & $63.5914 \pm 0.3309$ & $40.0656 \pm 0.5842$ & $58.9301 \pm 0.4422$ \\
\bottomrule
\end{tabular}
\centering
\caption{Kaggle FastText}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{easy} & \multicolumn{2}{c}{hard}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $55.9782 \pm 0.4295$ & $79.6147 \pm 0.0971$ & $47.4258 \pm 0.2784$ & $70.9725 \pm 0.0663$ \\
IDF & NN &  $57.6907 \pm 0.3138$ & $82.8576 \pm 0.0821$ & $49.1503 \pm 0.2648$ & $73.8446 \pm 0.2201$ \\
\midrule
AVG & Proto &  $59.0944 \pm 0.8332$ & $68.1744 \pm 0.8831$ & $49.6979 \pm 0.8749$ & $60.7554 \pm 1.8041$ \\
IDF & Proto &  $63.2457 \pm 0.8334$ & $76.2969 \pm 0.5677$ & $53.4766 \pm 0.7616$ & $65.2547 \pm 0.6531$ \\
CNN & Proto &  $64.7452 \pm 1.8330$ & $72.6063 \pm 3.8176$ & $49.7233 \pm 1.6391$ & $58.8577 \pm 3.5117$ \\
\midrule
AVG & MAML &  $37.0695 \pm 1.7642$ & $45.7326 \pm 1.0947$ & $29.4002 \pm 0.6920$ & $33.9531 \pm 0.9490$ \\
IDF & MAML &  $41.7356 \pm 1.3908$ & $49.5818 \pm 1.2517$ & $32.2761 \pm 2.8328$ & $36.4192 \pm 1.8429$ \\
CNN & MAML &  $38.1998 \pm 2.6205$ & $40.9244 \pm 2.5981$ & $30.6651 \pm 1.4987$ & $30.8549 \pm 1.3415$ \\
\midrule
AVG & R2D2 &  $62.8867 \pm 0.5169$ & $89.4721 \pm 0.1411$ & $52.8576 \pm 0.1536$ & $83.9281 \pm 0.2247$ \\
IDF & R2D2 &  $69.4593 \pm 1.5271$ & $92.6750 \pm 0.1200$ & $58.7341 \pm 1.2269$ & $86.9517 \pm 0.0518$ \\
CNN & R2D2 &  $72.3916 \pm 1.4550$ & $88.4818 \pm 0.3559$ & $56.1536 \pm 1.7958$ & $78.4020 \pm 1.1144$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $77.9733 \pm 1.1537$ & $94.5813 \pm 0.4311$ & $\bm{65.4256} \pm 0.5012$ & $88.3461 \pm 0.5542$ \\
\multicolumn{2}{l}{Ours} &  $\bm{80.6023} \pm 0.9371$ & $\bm{95.6779} \pm 0.1381$ & $64.7738 \pm 2.1268$ & $\bm{89.2747} \pm 0.6618$ \\
\multicolumn{2}{l}{Ours+fuse} &  $79.7517 \pm 1.0569$ & $95.7403 \pm 0.2674$ & $66.8171 \pm 0.5870$ & $89.8645 \pm 0.3190$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $81.7002 \pm 0.5611$ & $96.0017 \pm 0.1496$ & $67.9883 \pm 0.4651$ & $89.8822 \pm 0.4682$ \\
\bottomrule
\end{tabular}
\centering
\caption{Reuters FastText}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{easy} & \multicolumn{2}{c}{hard}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $60.1604 \pm 0.4783$ & $78.6960 \pm 0.2051$ & $43.7686 \pm 0.1483$ & $60.8429 \pm 0.1977$ \\
IDF & NN &  $57.1876 \pm 0.5613$ & $76.7600 \pm 0.2158$ & $41.9619 \pm 0.2213$ & $58.2701 \pm 0.2304$ \\
\midrule
AVG & MAML &  $30.3122 \pm 0.9289$ & $38.5803 \pm 1.6080$ & $28.4863 \pm 0.9647$ & $31.2240 \pm 1.5318$ \\
IDF & MAML &  $35.1080 \pm 1.0187$ & $44.5968 \pm 1.2381$ & $32.1425 \pm 0.5167$ & $35.6312 \pm 0.8350$ \\
CNN & MAML &  $28.5684 \pm 1.2994$ & $32.6491 \pm 0.7719$ & $28.4394 \pm 0.6894$ & $29.3312 \pm 0.8184$ \\
\midrule
AVG & Proto &  $50.8173 \pm 1.3621$ & $64.7605 \pm 1.1243$ & $43.4817 \pm 0.4354$ & $55.7291 \pm 0.9595$ \\
IDF & Proto &  $52.7109 \pm 1.6783$ & $67.1792 \pm 0.9993$ & $43.1777 \pm 1.1595$ & $56.5739 \pm 0.9273$ \\
CNN & Proto &  $45.0880 \pm 1.7562$ & $56.0240 \pm 1.4381$ & $37.2556 \pm 1.0012$ & $45.9280 \pm 1.3240$ \\
\midrule
AVG & R2D2 &  $65.5710 \pm 0.3759$ & $86.5773 \pm 0.3006$ & $48.1722 \pm 0.1778$ & $72.6245 \pm 0.1799$ \\
IDF & R2D2 &  $66.9684 \pm 1.0216$ & $\bm{87.5821} \pm 0.2632$ & $48.6552 \pm 0.5784$ & $72.8515 \pm 0.2141$ \\
CNN & R2D2 &  $53.4242 \pm 1.0365$ & $70.4477 \pm 0.7993$ & $41.8183 \pm 1.4924$ & $59.4736 \pm 0.5882$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $66.3636 \pm 0.7808$ & $86.5608 \pm 0.2660$ & $51.5139 \pm 0.7485$ & $75.3451 \pm 0.9706$ \\
\multicolumn{2}{l}{Ours} &  $\bm{69.2046} \pm 0.9465$ & $87.4267 \pm 0.2607$ & $\bm{54.1476} \pm 1.0628$ & $\bm{75.3885} \pm 1.1277$ \\
\multicolumn{2}{l}{Ours+fuse} &  $70.3859 \pm 1.0401$ & $88.0560 \pm 0.2048$ & $55.2337 \pm 1.1001$ & $76.2461 \pm 0.5291$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $70.2364 \pm 1.3098$ & $88.1493 \pm 0.1632$ & $55.0627 \pm 0.6474$ & $75.2384 \pm 0.5345$ \\
\bottomrule
\end{tabular}
\centering
\caption{RCV1 FastText}
\end{table*}

\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{Easy} & \multicolumn{2}{c}{Hard}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding &1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $23.2370 \pm 0.2043$ & $34.2298 \pm 0.2848$ & $23.6800 \pm 0.1501$ & $33.5698 \pm 0.1892$ \\
IDF & NN &  $33.4952 \pm 0.1859$ & $45.7150 \pm 0.1743$ & $32.3440 \pm 0.1909$ & $41.8882 \pm 0.2588$ \\
\midrule
AVG & Proto &  $34.2112 \pm 0.5664$ & $49.7726 \pm 1.9037$ & $27.0818 \pm 0.2761$ & $38.2938 \pm 0.6299$ \\
IDF & Proto &  $36.0683 \pm 0.8495$ & $54.5885 \pm 0.9925$ & $28.0243 \pm 0.5926$ & $41.9118 \pm 1.7005$ \\
CNN & Proto &  $36.1702 \pm 1.0072$ & $50.5523 \pm 0.9611$ & $27.5010 \pm 0.7425$ & $36.5462 \pm 0.9478$ \\
\midrule
AVG & MAML &  $35.6862 \pm 2.2598$ & $47.5048 \pm 0.5288$ & $26.0402 \pm 0.5419$ & $33.6421 \pm 0.3829$ \\
IDF & MAML &  $38.7443 \pm 0.7182$ & $50.3440 \pm 0.5765$ & $27.8302 \pm 0.4070$ & $36.4672 \pm 0.5190$ \\
CNN & MAML &  $36.4646 \pm 0.8876$ & $45.1965 \pm 1.2255$ & $25.2603 \pm 0.6605$ & $30.5365 \pm 0.7629$ \\
\midrule
AVG & R2D2 &  $25.3482 \pm 0.1450$ & $51.5232 \pm 0.1418$ & $25.5907 \pm 0.1319$ & $48.7152 \pm 0.2102$ \\
IDF & R2D2 &  $40.3838 \pm 0.1152$ & $61.7267 \pm 1.0365$ & $37.7374 \pm 0.1638$ & $55.8837 \pm 0.9760$ \\
CNN & R2D2 &  $41.3725 \pm 0.5487$ & $53.1038 \pm 0.7608$ & $30.8450 \pm 0.3336$ & $40.3256 \pm 0.9353$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $41.8048 \pm 0.1570$ & $62.5174 \pm 0.7638$ & $\bm{38.9325} \pm 0.3088$ & $57.1043 \pm 0.7719$ \\
\multicolumn{2}{l}{Ours}  &  $\bm{42.1267} \pm 0.1568$ & $\bm{62.9709} \pm 0.6772$ & $38.9002 \pm 0.1413$ & $\bm{57.3115} \pm 0.7644$ \\
\multicolumn{2}{l}{Ours+fuse} &  $42.5350 \pm 0.1749$ & $63.8587 \pm 0.1168$ & $39.1333 \pm 0.2211$ & $58.3987 \pm 0.2867$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $42.5581 \pm 0.1670$ & $64.0138 \pm 0.1065$ & $39.0829 \pm 0.2574$ & $58.1115 \pm 0.4213$ \\
\bottomrule
\end{tabular}
\centering
\caption{Kaggle BERT (We should put this table in appendix, because BERT is not that useful for topic classification.}
\end{table*}


\begin{table*}[h]
\small
\begin{tabular}{llcccc}
\toprule
\multicolumn{2}{c}{Model}& \multicolumn{2}{c}{easy} & \multicolumn{2}{c}{hard1}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
classifier & embedding & 1 shot & 5 shot & 1 shot & 5 shot\\
\midrule
AVG & NN &  $55.3317 \pm 0.2495$ & $69.8454 \pm 0.2906$ & $52.3792 \pm 0.2716$ & $64.8512 \pm 0.2554$ \\
IDF & NN &  $50.4168 \pm 0.3007$ & $66.0114 \pm 0.2811$ & $48.6544 \pm 0.1857$ & $62.3544 \pm 0.1875$ \\
\midrule
AVG & Proto &  $66.1291 \pm 1.7882$ & $78.8344 \pm 0.8779$ & $50.2781 \pm 0.9861$ & $66.2482 \pm 2.0124$ \\
IDF & Proto &  $63.5270 \pm 1.5752$ & $78.7155 \pm 0.6817$ & $48.2387 \pm 0.5850$ & $67.8245 \pm 0.7222$ \\
CNN & Proto &  $73.3688 \pm 1.7426$ & $84.1232 \pm 0.8571$ & $57.0867 \pm 5.5289$ & $75.0168 \pm 2.2109$ \\
\midrule
AVG & MAML &  $69.2824 \pm 0.3854$ & $73.7442 \pm 1.0092$ & $37.6827 \pm 2.0435$ & $50.0453 \pm 3.1713$ \\
IDF & MAML &  $67.9002 \pm 1.2805$ & $73.0459 \pm 1.7411$ & $40.2526 \pm 2.0633$ & $51.8440 \pm 2.9404$ \\
CNN & MAML &  $68.9707 \pm 1.8266$ & $75.8674 \pm 1.2461$ & $53.1464 \pm 1.2640$ & $70.3219 \pm 1.7333$ \\
\midrule
AVG & R2D2 &  $60.0443 \pm 0.2282$ & $77.7810 \pm 0.2541$ & $55.6517 \pm 0.2770$ & $73.9115 \pm 0.7770$ \\
IDF & R2D2 &  $57.2587 \pm 0.2865$ & $76.3922 \pm 0.2709$ & $54.4867 \pm 0.2627$ & $73.4894 \pm 0.7266$ \\
CNN & R2D2 &  $77.7626 \pm 0.4107$ & $86.6170 \pm 0.6184$ & $65.6531 \pm 5.7006$ & $78.6565 \pm 4.2490$ \\
\midrule
\multicolumn{2}{l}{Ours w/o $W_t$} &  $71.0803 \pm 0.2713$ & $85.8040 \pm 0.3161$ & $69.7667 \pm 0.7632$ & $87.8218 \pm 0.3604$ \\
\multicolumn{2}{l}{Ours} &  $71.1298 \pm 0.3506$ & $85.9514 \pm 0.2091$ & $70.0838 \pm 0.5696$ & $88.0734 \pm 0.2751$ \\
\multicolumn{2}{l}{Ours+fuse} &  $70.9200 \pm 0.3051$ & $85.7682 \pm 0.4343$ & $70.5365 \pm 0.6675$ & $88.1459 \pm 0.2533$ \\
\multicolumn{2}{l}{Ours+$w_{\text{idf}}$+fuse} &  $70.8096 \pm 0.1774$ & $75.7597 \pm 19.7265$ & $70.7261 \pm 0.4562$ & $88.3893 \pm 0.2514$ \\
\bottomrule
\end{tabular}
\centering
\caption{FewRel BERT. (This result on the easy split is a little bit concerning. It seems that for the easy split, using lexicalized information helps, athere are overlaps between train and test.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{llccc}
\toprule
Samples & Way & Acc\\
\midrule
1       & 5     & $0.3833 \pm 0.0420$\\
5       & 5     & $0.7057 \pm 0.0526$\\
10      & 5     & $0.7932 \pm 0.0357$\\
15      & 5     & $0.8311 \pm 0.0279$ \\
20      & 5     & $0.8535 \pm 0.0316$ \\
25      & 5     & $0.8675 \pm 0.0316$ \\
50      & 5     & $0.8940 \pm 0.0249$ \\
100     & 5     & $0.9164 \pm 0.0235$ \\
200     & 5     & $0.9355 \pm 0.0152$ \\
300     & 5     & $0.9436 \pm 0.0128$ \\
\bottomrule
\end{tabular}
\caption{20 Newsgroups.}
\end{table*}

\begin{table*}[t!]
\centering
\begin{tabular}{llccc}
\toprule
Samples & Way & Acc\\
\midrule
1       & 5     & $0.3968 \pm 0.0720$ \\
5       & 5     & $0.6700 \pm 0.0445$ \\
10      & 5     & $0.7255 \pm 0.0450$ \\
15      & 5     & $0.7644 \pm 0.0386$ \\
20      & 5     & $0.7791 \pm 0.0302$ \\
25      & 5     & $0.7928 \pm 0.0297$ \\
50      & 5     & $0.8246 \pm 0.0308$ \\
100     & 5     & $0.8498 \pm 0.0289$ \\
200     & 5     & $0.8648 \pm 0.0224$ \\
300     & 5     & $0.8715 \pm 0.0242$ \\
500     & 5     & $0.8809 \pm 0.0237$ \\
\bottomrule
\end{tabular}
\caption{Amazon.}
\end{table*}


==> section/tables/lmi-amazon.tex <==
\begin{table*}[t]
\tiny
\begin{tabular}{cccccccc}
\toprule
\emph{Amazon Instant Video}&\emph{Apps for Android}&\emph{Automotive}   &\emph{Baby}         &\emph{Beauty}       &\emph{Books}        \\
\midrule
season       &app          &car          &baby         &skin         &book         \\
series       &kindle       &wax          &tub          &hair         &circus       \\
episode      &game         &filter       &bottles      &face         &read         \\
episodes     &apps         &oil          &potty        &product      &story        \\
watch        &free         &battery      &diaper       &dry          &jacob        \\
seasons      &android      &vehicle      &son          &moisturizer  &characters   \\
shows        &calories     &product      &gate         &acne         &life         \\
watching     &play         &engine       &crib         &use          &novel        \\
characters   &radio        &use          &diapers      &using        &reading      \\
tv           &phone        &paint        &bottle       &lotion       &gruen        \\
\midrule
\midrule
\emph{CDs and Vinyl}&\emph{Cell Phones and Accessories}&\emph{Clothing Shoes and Jewelry}&\emph{Digital Music}&\emph{Electronics}  &\emph{Grocery and Gourmet Food}\\
\midrule
dvd          &phone        &wear         &quot         &headphones   &tea          \\
concert      &headset      &bra          &album        &sound        &taste        \\
video        &charger      &size         &songs        &koss         &flavor       \\
music        &ear          &fit          &cd           &nook         &coffee       \\
film         &bluetooth    &shoes        &song         &radio        &sauce        \\
songs        &charge       &pair         &music        &bass         &sugar        \\
album        &case         &jeans        &albums       &pair         &chocolate    \\
quot         &battery      &comfortable  &track        &camera       &hot          \\
band         &motorola     &wearing      &tracks       &ear          &milk         \\
movie        &usb          &pants        &lyrics       &cable        &cup          \\
\midrule
\midrule
\emph{Health and Personal Care}&\emph{Home and Kitchen}&\emph{Kindle Store} &\emph{Movies and TV}&\emph{Musical Instruments}&\emph{Office Products}\\
\midrule
brush        &oxo          &book         &movie        &guitar       &labels       \\
razor        &ice          &story        &film         &strings      &tape         \\
product      &cream        &read         &jesus        &sound        &paper        \\
batteries    &bowl         &author       &dvd          &pedal        &avery        \\
shave        &handle       &characters   &christ       &picks        &ink          \\
skin         &kitchen      &books        &movies       &string       &printer      \\
use          &salad        &series       &watch        &guitars      &print        \\
shaver       &use          &reading      &mel          &mic          &label        \\
clean        &opener       &kindle       &films        &strap        &folders      \\
braun        &potatoes     &stories      &godzilla     &acoustic     &use          \\
\midrule
\midrule
\emph{Patio Lawn and Garden}&\emph{Pet Supplies} &\emph{Sports and Outdoors}&\emph{Tools and Home Improvement}&\emph{Toys and Games}&\emph{Video Games}  \\
\midrule
deer         &dog          &knife        &saw          &game         &game         \\
trap         &food         &cleaning     &blade        &fun          &games        \\
garden       &dogs         &gun          &tool         &play         &graphics     \\
squirrels    &water        &bore         &table        &cards        &play         \\
yard         &cat          &patches      &dewalt       &kids         &fun          \\
feeder       &tank         &barrel       &router       &pieces       &played       \\
plants       &filter       &use          &cut          &board        &gameplay     \\
sprayer      &cats         &knives       &wood         &games        &dreamcast    \\
grill        &fish         &belt         &dust         &toy          &mario        \\
traps        &toy          &rod          &drill        &players      &playing      \\
\bottomrule
\end{tabular}
\centering
\caption{Top 10 LMI-ranked words for each class in Amazon.
  Class names are shown in italic.  }\label{tab:lmi_amazon}
\end{table*}


==> section/tables/tab-bert.tex <==
\begin{table}[t]
\small
\begin{tabular}{llcccccc}
\toprule
\multicolumn{2}{c}{Method}& \multicolumn{2}{c}{HuffPost} & \multicolumn{2}{c}{FewRel}\\
\cmidrule(lr{0.5em}){1-2}\cmidrule(lr{0.5em}){3-4}\cmidrule(lr{0.5em}){5-6}
Rep. & Alg. & 1 shot & 5 shot & 1 shot & 5 shot \\
\midrule
\textsc{avg} &\textsc{nn} &$23.23  $ & $34.22  $ & $52.37  $ & $64.85  $ \\
\textsc{idf} &\textsc{nn} &$33.49  $ & $45.71  $ & $48.65  $ & $62.35  $ \\
\textsc{cnn} &\textsc{ft} &$37.30  $ & $51.56  $ & $61.10$  & $80.04$ \\
\midrule
\textsc{avg} &\textsc{proto} &$34.21  $ & $49.77  $ & $50.27  $ & $66.24  $ \\
\textsc{idf} &\textsc{proto} &$36.06  $ & $54.58  $ & $48.23  $ & $67.82  $ \\
\textsc{cnn} &\textsc{proto} &$36.17  $ & $50.55  $ & $57.08  $ & $75.01  $ \\
\midrule
\textsc{avg} &\textsc{maml} &$35.68  $ & $47.50  $ & $37.68  $ & $50.04  $ \\
\textsc{idf} &\textsc{maml} &$38.74  $ & $50.34  $ & $40.25  $ & $51.84  $ \\
\textsc{cnn} &\textsc{maml} &$36.46  $ & $45.19  $ & $53.14  $ & $70.32  $ \\
\midrule
\textsc{avg} &\textsc{rr}& $25.34  $ & $51.52  $ & $55.65  $ & $73.91  $ \\
\textsc{idf} &\textsc{rr} & $40.38  $ & $61.72  $ & $54.48  $ & $73.48  $ \\
\textsc{cnn} &\textsc{rr} &$41.37  $ & $53.10  $ & $65.65  $ & $78.65  $ \\
\midrule
\textsc{our} & \textsc{rr} & $\bm{42.12}  $ & $\bm{62.97}  $ & $\bm{70.08}  $ & $\bm{88.07}  $ \\
\bottomrule
\end{tabular}
\centering
\caption{5-way 1-shot and 5-way 5-shot classification
on HuffPost and FewRel using BERT.
(See Table~\ref{tab:bert-std} in Appendix~\ref{app:result} for standard deviations.)}\label{tab:bert}
\end{table}

